A Practical and Secure Byzantine Robust Aggregator

In machine learning security, one is often faced with the problem of removing outliers from a given set of high-dimensional vectors when computing their average. For example, many variants of data poisoning attacks produce gradient vectors during training that are outliers in the distribution of clean gradients, which bias the computed average used to derive the ML model. Filtering them out before averaging serves as a generic defense strategy. Byzantine robust aggregation is an algorithmic primitive which computes a robust average of vectors, in the presence of an $\epsilon$ fraction of vectors which may have been arbitrarily and adaptively corrupted, such that the resulting bias in the final average is provably bounded. In this paper, we give the first robust aggregator that runs in quasi-linear time in the size of input vectors and provably has near-optimal bias bounds. Our algorithm also does not assume any knowledge of the distribution of clean vectors, nor does it require pre-computing any filtering thresholds from it. This makes it practical to use directly in standard neural network training procedures. We empirically confirm its expected runtime efficiency and its effectiveness in nullifying 10 different ML poisoning attacks.

==> sections/discussion.tex <==
\section{Discussion}

\subsection*{Circumventing Robust Aggregation}

Our findings show that a data poisoning attack is able to circumvent \randeigen  if and only if
the poisoned and clean samples are statistically indistinguishable (i.e. the assumptions of Theorem 1
are not met). Under this condition, such attacks are still constrained bias the information-theoretic optimal
bias of $O(\sqrt{\epsilon ||\Sigma_S||_2)}$. Based on our evaluations, a bias of this magnitude does not significantly
impact the aggregated model's performance in the FL setup. Designing an attack which is able to 
subvert model performance within this bias bound is an interesting open problem for future work. 


\subsection*{Practical Considerations for Space Constraints}

Existing practical implementations of NO-REGRET and FILTERING over $d$-dimensional samples
 involve computing a $d \times d$ covariance matrix, which may require significant memory overhead if $d$ is large.
To address this, these implementations typically employ dimension-wise chunking, where each sample is split into $C$ chunks of
$\sim d/C$ dimensions each. However, this approach introduces a bias of of $O(\sqrt{C \epsilon ||\Sigma_S||_2})$ compounded across
chunks (similar to the case of dimension-wise aggregation). In contrast, RandEigen eliminates the need for chunking, by computing
the covariance matrix over $O(\log d)$ dimensions. 


 \subsection*{Dimensionality Reduction for Outlier Detection}

This work is, to our knowledge, the first to provide a theoretical foundation for leveraging Johnson-Lindenstrauss (JL) 
transforms in dimensionality reduction for efficient outlier detection.  
 While prior studies have empirically explored dimensionality reduction for outlier detection across various applications, 
our contribution formalizes this approach.
The problem of efficient outlier detection is of interest not only to the security community \cite{DBLP:conf/iclr/DuJS20, DBLP:journals/jnca/AhmedMH16}, 
but also to a other fields as well (see for example, \cite{DBLP:journals/csur/ChandolaBK09} for a survey).
Therefore, we envisage that this work will be of use to the broader statistics community in general.



==> sections/old_proofs.tex <==
\subsection{Textbook Approach}

\textit{Textbook assumes $(4\epsilon, \delta)$. For consistency, I use it here first. This section mainly follows the flow of Thm 2.17 of textbook}

We assume that the set of clean samples $S'$ is a $(4\epsilon, \delta)$-stable set. $X_0 := X$ is constructed by corrupting a $\epsilon$-fraction of samples from $S'$. Let $S_0 := S = S' \cap X$, $T_0:=T = X \setminus S$, and denote $X_i$ as the samples from $X$ remaining the beginning of the $i$-th iteration, $S_i = S \cap X_i$ and $T_i = X_i \setminus S_i$. Let $\mu_A$ and $\Sigma_A$ denote the empirical mean and covariance matrix of a set of samples $A$. Suppose Algorithm \ref{alg:filter_modified} runs for $\tau \in [1, 2n\epsilon]$ iterations

note: Update stopping condition in line 8 to be something like, terminate if the following holds: Let $N_i = |X_i| - \frac{1}{\max \mathcal{P}} \sum_{x \in X_i} |v \cdot(x - \mu_{X_i} ) | $. Terminate if $N_i \leq (1-3\epsilon)n$ and $|X_i| \leq (1-2\epsilon)n$. $N_i$ is the expected number of sample remaining after the current round of filtering. Informally, this means that we stop when the expected number of remaining samples if filtering is done this round is less than $(1-3\epsilon)n$ (or equivalently, the number of samples remaining in $S_i$ could drop below $(1-4\epsilon)n$)


\begin{assumption} \label{ass:textbook}
    Given an $\epsilon$-corrupted set $X$, constructed by corrupting an $\epsilon$-proportion of samples from a $(4\epsilon, \delta)$-stable set $S$ where $|S|=|X|=n$. X is said to satisfy the assumption if for all subsets $X' = S'\cup T'\subseteq X$ where $S' = X \cap S$ and $T' = X' \setminus S'$ and $|X'| \geq (1-4\epsilon)n$, the following holds:
        Let $v$ be the dominant eigenvector of $\Sigma_{X'}$. The following holds: 
        \begin{equation} \label{eqn:textbook_ass}
    \sum_{t \in T'} |v\cdot (t - \mu_{X'})| \geq \sum_{s \in S'} |v\cdot (s - \mu_{X'})|.
    \end{equation}
\end{assumption}




\begin{lemma} \label{lemma:doob_maximal_ineq}
    [\emph{Proposition A.5 of \cite{diakonikolas2023algorithmic}}]
    Let $M_1, \dots, M_n$ be a sequence of supermartingales, where $M_i \geq 0$ a.s. for all $i$. Then, for all $\zeta \geq 1,$ $\IP[\max_{1 \leq i \leq n} X_i \geq \zeta \IE[M_1]] \leq \frac{1}{\zeta}$ 
\end{lemma}
We omit the proof for Lemma \ref{lemma:doob_maximal_ineq}, as it is a well-known result in martingale theory (Doob's maximal inequality). The exact proof is given in Proposition A.5 of \cite{diakonikolas2023algorithmic}.


\begin{lemma} \label{lemma:min_size_xi}
    Let $X$ be a $\epsilon$-corrupted version of a $(4\epsilon, \delta)$-stable set $S$ and assume that $X$ satisfies Assumption \ref{ass:textbook}. Let $X_i$ be the samples remaining at the beginning of the $i$-th iteration when Algorithm \ref{alg:filter_modified} is performed on $X$. When Algorithm \ref{alg:filter_modified} terminates at $\tau$ iterations, 
    $|X_\tau \cap S| \geq (1-4\epsilon)n$ with probability at least $\frac{2}{3}$
\end{lemma}

\begin{proof}

    (note: this incorporates the modified line 9)
    There are three possible stopping conditions of Algorithm \ref{alg:filter_modified}: Lines 2, 3 and 9. If the algorithm terminates at Line 9, the number of samples is in $X_\tau$ is at least $(1-3\epsilon)n$. Since $|T_i| \leq \epsilon n$, it follows that $|X_\tau \cap S| \geq (1-4\epsilon)n$ with probability 1. Thus, we consider the other two stopping conditions in the subsequent proof.  




    Define $d(X_i) = |T_i| + |S \setminus S_i|$, which is the sum of the number of corrupted samples remaining and the total number of clean samples removed at the beginning of iteration $i$. Note that $d(X_0) \leq \epsilon n$, and $d(X_i) \geq 0$ for all $i$. The role of $d(X_i)$ is as follows: if $d(X_i)$ is a decreasing sequence in expectation (i.e. a supermartingale), the number of samples removed from $T_i$ exceeds those removed from $S_i$ in expectation. 

    Let $\max \mathcal{P}$ be as defined in Line 12 of Algorithm \ref{alg:filter_modified}, and consider $H(X_{i+1}) = d(X_{i+1}) - d(X_i)$, which is the number of samples from $S_i$ removed at the $i$-th iteration, subtracted by the number of samples from $T_i$ removed at the $i$-th iteration. Then,
    \[
    \begin{split}
    \IE[H(X_i+1)] & = \frac{1}{\max \mathcal P} \left[-\sum_{t \in T'} |v\cdot (t - \mu_{X_i})| + \sum_{s \in S'} |v\cdot (s - \mu_{X_i})| \right] \\
    &\leq 0
    \end{split}
    \]
    where the final bound is due to Assumption \ref{ass:textbook} (\ref{eqn:textbook_ass}). Since $\IE[H(X_i+1)] \leq 0$, the sequence of $d(X_i)$'s are supermartingales as long as Assumption \ref{ass:textbook} is satisfied. 
    
    It remains to bound $|S_0 \setminus S_\tau|$, which is the number of samples removed throughout the $\tau$ iterations. Note that $|S_0 \setminus S_\tau| \leq d(X_\tau)$, $\IE[d(X_0)] \leq n\epsilon$ and $d(X_i) \geq 0$.
    Setting $M_i = d(X_i)$ and applying Doob's maximal inequality (Lemma \ref{lemma:doob_maximal_ineq}), $\IP[d(S_\tau) \geq 3\epsilon n] \leq \leq \IP[d(S_\tau) \geq 3\IE[d(X_0)] ] \leq \frac{1}{3}$ or equivalently, $\IP[d(S_\tau) < 3\epsilon n] > \frac{2}{3}$. Thus, $\IP[|S_0 \setminus S_\tau| < 3\epsilon n] > \frac{2}{3}$. Finally, since $|S_0| \geq (1-\epsilon)n$, $\IP[|X_\tau \cap S| \geq (1-4\epsilon)n] \geq \frac{2}{3}$. 
\end{proof}


\begin{lemma}\label{lemma:ei_decrease}

    Let $X$ be a $\epsilon$-corrupted version of a $(4\epsilon, \delta)$-stable set $S$. Let $X_i$ be the samples remaining at the beginning of the $i$-th iteration when Algorithm \ref{alg:filter_modified} is performed on $X$. 
   Define $\epsilon_i = \frac{|T_i|}{|X_i|}$. 
    If $X$ satisfies Assumption \ref{ass:textbook},
    then, $\IE[\epsilon_{i+1}|X_i] < \epsilon_i$ with probability at least $\frac{2}{3}$.
\end{lemma}
\begin{proof}

    By Lemma \ref{lemma:min_size_xi}, $|X_i| \geq (1-4\epsilon)n$. Thus, by assumption, $X_i$ satisfies the properties in Assumption \ref{ass:textbook}.
    
    Consider the ratio $R_i = \frac{|T_i|}{|S_i|}$. Since the removal of samples in $X_i$ in a fixed iteration are independent events, $|T_i|$ and $|S_i|$ are independent. 
    Thus, 
    \[
        \IE \left[\frac{|T_{i+1}|}{|S_{i+1}|} \middle| X_i \right] = \IE \left[\frac{|T_{i}| - |T_i \setminus T_{i+1}|}{|S_{i}| - |S_i \setminus S_{i+1}|} \middle| X_i \right]  = \frac{|T_i| - \IE[|T_i \setminus T_{i+1}||X_i]}{|S_{i}| - \IE[|S_i \setminus S_{i+1}|X_i]}.
    \]
    By Assumption \ref{ass:textbook} (\ref{eqn:textbook_ass}),
    \begin{equation} \label{eqn:ti_si_bound}
    \begin{split}
    \IE[|T_i \setminus T_{i+1}||X_i] & = \frac{1}{\max \mathcal{P}} \sum_{t \in T'} |v\cdot (t - \mu_{X'})| \\
    & \geq \frac{1}{\max \mathcal{P}}  \sum_{s \in S'} |v\cdot (s - \mu_{X'})| =  \IE[|S_i \setminus S_{i+1}|X_i].
    \end{split}
    \end{equation}
    Since $|T_i| < |S_i|$ and (\ref{eqn:ti_si_bound}), 
    \[
    \IE \left[\frac{|T_{i+1}|}{|S_{i+1}|} \middle| X_i \right] =\frac{|T_i| - \IE[|T_i \setminus T_{i+1}||X_i]}{|S_{i}| - \IE[|S_i \setminus S_{i+1}|X_i]} < \frac{|T_i|}{|S_i|}.
    \]
    Thus, 
    \[
       \frac{1}{\IE[\epsilon_{i+1}|X_i]} \stackrel{(*)}{\leq} \IE\left[\frac{1}{\epsilon_{i+1}} \middle| X_i\right] =\IE \left[1+\frac{|T_{i+1}|}{|S_{i+1}|} \middle| X_i \right]  < 1+ \frac{|T_i|}{|S_i|} = \frac{1}{\epsilon_i},
    \]
    where we applied Jensen's inequality in (*). Thus, 
    $\IE[\epsilon_{i+1}|X_i] < \epsilon_i$. 
\end{proof}



\begin{lemma}\label{lemma:eigenvalue_converge}
    Suppose Algorithm \ref{alg:filter_modified} terminates at $\tau \leq 2n\epsilon$
    iterations. Then, the sequence of values $||\Sigma_{X_i}||_2 - ||\Sigma_{I_i}||_2$ converges to 0, for $i=1, \dots, \tau$ with probability at least $\frac{2}{3}$. 
\end{lemma}

\begin{proof}
        The following is an algebraic fact (also used in the original analysis of~\cite{diakonikolas2023algorithmic})):
    \begin{equation} \label{eqn:sigma_xi_converge}
        \Sigma_{X_i} = (1-\epsilon_i) \Sigma_{I_i} + \epsilon_i \Sigma_{O_i} + \epsilon_i (1-\epsilon_i) (\mu_{O_i} - \mu_{I_i})(\mu_{O_i} - \mu_{I_i})^T,
    \end{equation}

    By Lemma \ref{lemma:ei_decrease}, the proportion of corrupted samples $\epsilon_i = \frac{|T_i|}{|X_i|}$ is a strictly decreasing sequence with probability at least $\frac{2}{3}$. Thus, the terms in (\ref{eqn:sigma_xi_converge}) which are proportional to $\epsilon_i$ are decreasing and converging to 0
    in expectation, while $(1-\epsilon_i) \Sigma_{S_i}$ is converging to $\Sigma_{X_i}$. Thus, 
    $\Sigma_{X_i}$ is converging to $\Sigma_{S_i}$, or equivalently, $||\Sigma_{X_i}||_2 - ||\Sigma_{I_i}||$ converges to 0 when $\epsilon_i$ has converged to 0. 
    % Finally, at iteration $\tau$, since $|O_\tau|=0$, the sequence is no longer decreasing. 
\end{proof} 



\begin{theorem}
    Let $S$ be a $(4\epsilon, \delta)$-stable set for some $\epsilon \leq \frac{1}{12}$, and construct $X$ by corrupting a $\epsilon$-fraction of points in $S$. Let $T = X \setminus S$. Assume that $X$ satisfies Assumption \ref{ass:textbook}. Then, Algorithm \ref{alg:filter_modified} terminates with a maximum bias of $\delta$ (to formalize the last sentence using our notations) with probability at least $\frac{2}{3}$. 
\end{theorem}

\begin{proof}
    By Lemma \ref{lemma:min_size_xi}, when Algorithm \ref{alg:filter_modified} terminates, there are at least $(1-4\epsilon)n$ samples remaining. 
    Remains to show that the bias of $|v\cdot (\mu_{X_\tau} - \mu_S)| \leq \delta$
    \begin{enumerate}
        \item (Convergence condition) By Lemma \ref{lemma:eigenvalue_converge}, the proportion of corrupted samples $\epsilon_i = \frac{|T_i|}{|X_i|}$ converges to 0 when this stopping condition is met. 
        \item (Counting condition). If this condition is satisfied, then at least $3\epsilon n$ samples from $X$ have been removed. On expectation, in every iteration, the number of samples removed from $T_i$ exceeds the number of samples removed from $S_i$. Thus, on expectation, all the $\epsilon n$ samples from $T$ have been removed, and at most $1.5\epsilon$ samples from $S$ have been removed. Therefore, the expected number of samples remaining in $S$ is $|S \cap X_\tau| \geq (1 - (1.5 +1)\epsilon) n = (1-2.5\epsilon)n$. (Formalize this in lemma)
        \item (Full $2n\epsilon$ iterations) Since each iteration removes at least one sample from $T_i$ on expectation (this is actually proven in the proof of Lemma \ref{lemma:min_size_xi}, i will make it a seperate lemma), then at $2n\epsilon$ iterations, all the $\epsilon n$ samples from $T$ should have been removed. 
    \end{enumerate}
    In all stopping condition, we showed that on expectation, all the samples from $T$ have been removed and $|S_\tau| > (1-4\epsilon)n$ with probability at least $\frac{2}{3}$. Thus, by stability,... 
\end{proof}


\subsection{old}
In Lemma \ref{lemma:eps_delta_max_bias}, we prove that any subset which consists of at least $1-\epsilon$ proportion of samples from a $(\epsilon, \delta)$-stable set $X$ has a bounded mean absolute deviation away from the sample mean of $X$. In Lemma \ref{lemma:inlier_filter_prob}, this mean absolute deviation will be used to compute the probability that a sample in $X$ is filtered out in Algorithm \ref{alg:filter_modified}. 



\begin{lemma} \label{lemma:outlier_filter_prob}
    Let $O_i$ be the set of outliers still remaining in
    the $i$-th iteration, as defined in (\ref{eqn:outlier_o}). Then, for all $o \in O_i$, 
    the probability that $o$ is filtered out in the $i$-th iteration is lower bounded by $ \sqrt{k||\Sigma_X||_2}/\max \mathcal{P}$, where $ \mathcal{P}$  is defined
    in Algorithm \ref{alg:filter_modified} (Line 8). 
\end{lemma}
\begin{proof}
    In (\ref{eqn:outlier_o}), a sample $o$ is deemed as an outlier if there exists a unit vector $v$, such that $|v \cdot(o - \mu_{x_i})| > \sqrt{k ||\Sigma_X||_2}$. 
    On the other hand, in Algorithm \ref{alg:filter_modified} (Line 12), $o$ is filtered
    out with probability $|v \cdot(o - \mu_{x_i})|/ \max \mathcal{P}$, which can be lower bounded by $ \sqrt{k||\Sigma_X||_2} / \max \mathcal{P}$
\end{proof}

\begin{lemma} \label{lemma:inlier_filter_prob}
    Let $I_i$ be the set of inlier still remaining in
    the $i$-th iteration, as defined in (\ref{eqn:inlier}). If $|I_i| \geq (1-\epsilon)n$, the expected proportion of inlier sample that  is filtered out is upper bounded by 
    $\frac{1}{\max \mathcal{P}} \sqrt{\frac{\delta^2}{\epsilon} + ||\Sigma_X||_2}$, where $ \mathcal{P}$  is defined
    in Algorithm \ref{alg:filter_modified} (Line 8).
\end{lemma}
\begin{proof}
    By Lemma \ref{lemma:eps_delta_max_bias}, since $I_i \subset X$
    \begin{equation} \label{eqn:ub_filter_inlier}
    \frac{1}{|I_i  |} \sum_{x\in I_i  } |v\cdot(x-\mu_X)|\leq \sqrt{\frac{\delta^2}{\epsilon} + ||\Sigma_X||_2}.
    \end{equation}
    In Algorithm \ref{alg:filter_modified} (Line 12), each $x\in I_i $ is filtered
    out with probability $|v\cdot(x-\mu_X)|/ \max \mathcal{P}$. 
    Thus, the expected number of samples filtered out is 
    $ \sum_{x\in I_i  }  \frac{1}{\max \mathcal{P}} |v\cdot(x-\mu_X)| $,
    Using the upper bound in (\ref{eqn:ub_filter_inlier}), the expected proportion of samples filtered out from $I_i$
    is upper bounded by, 
    \[
    \frac{1}{|I_i|}\sum_{x\in I_i  }  \frac{1}{\max \mathcal{P}} |v\cdot(x-\mu_X)| \leq \frac{1}{\max \mathcal{P}} \sqrt{\frac{\delta^2}{\epsilon} + ||\Sigma_X||_2}.
    \]
    
\end{proof}

In Lemma \ref{lemma:2eps}, we prove that in an $\epsilon$-corrupted set obtained by corrupting an $(\epsilon, \delta)$-stable set, there can be at most $2\epsilon$ proportion of outlier samples. Lemma \ref{lemma:natural_outlier} shows that at most  $\epsilon$-proportion of outliers are already present in the uncorrupted $(\epsilon, \delta)$-stable set, and an adversary could potentially replace an $\epsilon$-fraction of inlier samples while keeping the already present outliers.  

\begin{lemma} \label{lemma:natural_outlier}
    Let $S$ be a $(\epsilon, \delta)$-stable set of $n$ clean samples. For all $\epsilon' \leq \epsilon$,  there does not exist an $\epsilon'$ proportion of samples $S_{\epsilon'} \subset S$ where $|S_{\epsilon'}| = n \epsilon'$, and a unit vector $v$ s.t. $\frac{1}{|S_{\epsilon'}|}\left|\sum_{s \in S_{\epsilon'}} v \cdot(s - \mu_S) \right| > 2\frac{\delta}{{\epsilon'}}$.
\end{lemma}

\begin{proof} 
    Suppose there exists a $S_{\epsilon'} \subset S$ where $|S_{\epsilon'}| = n \epsilon'$ for some $\epsilon' \leq \epsilon$, and a unit vector $v$ where $\frac{1}{n\epsilon'}\left|\sum_{s \in S_{\epsilon'}} v \cdot(s - \mu_S) \right| > 2\frac{\delta}{\epsilon'}$. Without loss of generality, suppose that 
    $\frac{1}{|S_{\epsilon'}|}\sum_{s \in S_{\epsilon'}} v \cdot(s - \mu_S)  > 2\frac{\delta}{\epsilon'}$.
    
    By the $(\epsilon, \delta)$ stability of $S$ (Definition \ref{dfn:epsilon_delta_stable} (1)), since $|S \setminus S_{\epsilon'}| = (1-\epsilon')n \geq (1-\epsilon)n$,  $\frac{1}{(1-\epsilon')n}\left|\sum_{x \in S \setminus S_{\epsilon'}} v \cdot(s - \mu_S) \right| \leq \delta$. Thus, 
    \[
    \begin{split}
        \frac{1}{n} \left|\sum_{y \in S} v\cdot(y - \mu_S) \right| &=  \frac{1}{n} \left|\sum_{s \in S_{\epsilon'}} v \cdot(s - \mu_S) + \sum_{x \in S \setminus S_{\epsilon'}} v \cdot(s - \mu_S)  \right| \\
        & \geq \frac{1}{n} \left(n\epsilon' \left(2 \frac{\delta}{\epsilon'} \right) + n(1-\epsilon') (-\delta) \right) \\
        & \geq 2\delta + (1-\epsilon')(-\delta) \\
        & = \delta (1+\epsilon') > \delta,
    \end{split}
    \]
    which violates the $(\epsilon, \delta)$ stability of $S$ (Definition \ref{dfn:epsilon_delta_stable} (1)).
\end{proof}
\begin{lemma} \label{lemma:2eps}
    Let $O_0$ be the set of outlier samples before the start of the first iteration, as defined in (\ref{eqn:outlier_o}). Then, $|O_0| \leq 2n\epsilon$.
\end{lemma}
\begin{proof}
    By Lemma \ref{lemma:natural_outlier}, for all $\epsilon' < \epsilon$, no $\epsilon'$-fraction of samples from the set of clean samples exists such that the mean computed over these samples deviates from the overall sample mean of all clean samples by more than $2\frac{\delta}{\epsilon'}$ in any direction.

    During corruption, an adversary can corrupt up to an additional $\epsilon$ proportion of the clean samples. Consequently, the proportion of outliers in the $\epsilon$-corrupted set is at most $2\epsilon$. Hence,  $|O_\tau| \leq 2\epsilon n$.
\end{proof}

In Lemma \ref{lemma:ri}, we show that the ratio of the number of outlier samples to inlier samples is decreasing in expectation with each iteration, if the condition given in Lemma \ref{lemma:k} is fulfilled. 
\begin{lemma} \label{lemma:ri}
    Let $r_i$ denote the ratio of outliers
    to inliers $\frac{|O_i|}{|I_i|}$
    at the end of the $i$-th iteration. Then, 
    \begin{equation} 
    \IE[r_{i}|r_{i-1}] \leq r_{i-1} \exp\left(-\frac{1}{\max \mathcal{P}}  \left( \sqrt{ ||\Sigma_X||_2} \left(\sqrt{k}- \sqrt{\frac{20}{\epsilon} + 1} \right) \right)\right),
    \end{equation}
    where $\max \mathcal{P}$ is as defined in Line 8 of Algorithm \ref{alg:filter_modified}. 
\end{lemma}

\begin{proof}
    We first express $r_i$ in terms of $r_{i-1}$. Let
    $A_i$ and $B_i$ denote the proportion of outliers
    and inliers that remain after the $i$-th iteration (w.r.t. $|O_i|$ and $|I_i|$), respectively, which are independent for any fixed $i$. 
    \[
    \begin{split}
        r_i &= \frac{|O_i|}{|I_i|}
        =\frac{|O_{i-1}|}{|I_{i-1}|} \frac{A_{i-1}}{B_{i-i}}
        = r_{i-1} \frac{A_{i-1}}{B_{i-i}}.
    \end{split}
    \]
    Thus, we have
    \begin{equation}\label{eqn:ri_ri-1}
    \begin{split}
        \IE[r_i|r_{i-1}] = \IE \left[ r_{i-1} \frac{A_{i}}{B_{i}} \middle| r_{i-1}\right] = r_{i-1}  \frac{\IE[A_{i}|r_{i-1}]}{\IE[B_{i}|r_{i-1}]},
    \end{split}
    \end{equation}
    where  $\IE\left[\frac{A_i}{B_i}\middle|r_{i-1}\right]=\frac{\IE[A_{i}|r_{i-1}]}{\IE[B_{i}|r_{i-1}]}$, as $A_i$ and $B_i$ are cond. independent.

    By Lemma \ref{lemma:outlier_filter_prob},
    the probability that an outlier sample is filtered out is lower bounded by $\frac{\sqrt{k||\Sigma_X||_2}}{\max \mathcal{P}}$. By Lemma \ref{lemma:2eps}, $|O_{i-1}| \leq |O_0| = 2n\epsilon$. Thus, by linearity of expectation, 
    \[
    \begin{split}
    \IE_{i-1}[|O_{i-1} \setminus O_i|] &= \sum_{o \in O_i} \IE_{i-1}[\text{$o$ is filtered out}]\\
    & \geq \sum_{o \in O_i} \frac{ \sqrt{k||\Sigma_X||_2}}{\max \mathcal{P}} \\
    &= |O_{i-1}| \frac{ \sqrt{k||\Sigma_X||_2}}{\max \mathcal{P}}.
    \end{split}
    \]
    Hence, 
\[
\begin{split}
    \IE_{i-1}[A_i] & = 1-\frac{\IE_{i-1}[|O_{i-1} \setminus O_i|]}{|O_{i-1}|} \\
    & \leq 1- \frac{ \sqrt{k ||\Sigma_X||_2}}{\max \mathcal{P}}\\
   & \approx \exp \left(- \frac{ \sqrt{k ||\Sigma_X||_2}}{\max \mathcal{P}}  \right),
\end{split}
\]
where we used the approximation $1-x \approx \exp(-x)$ in the last step, for small $x$. In this case, since $\max \mathcal{P}$ is computed over the outlier samples, $\max \mathcal{P} \gg  \sqrt{k ||\Sigma_X||_2}$, and thus,  $\frac{ \sqrt{k ||\Sigma_X||_2}}{\max \mathcal{P}} $ is close to $0$.
Similarly, by Lemma \ref{lemma:inlier_filter_prob}, 
    \[
    \begin{split}
        \IE_{i-1}[B_i] & \geq 1-\frac{1}{\max \mathcal{P}} \sqrt{\frac{\delta^2}{\epsilon} + ||\Sigma_X||_2} \\
        &\approx \exp \left(-\frac{1}{\max \mathcal{P}} \sqrt{\frac{\delta^2}{\epsilon} + ||\Sigma_X||_2}\right).
    \end{split}
    \]
    Since $\delta = \sqrt{20 ||\Sigma_X||_2}$, 
    \begin{equation}\label{equation:ratio}
    \begin{split}
        \frac{\IE_{i-1}[A_{i}]}{\IE_{i-1}[B_{i}]} & \leq \frac{1- \frac{\sqrt{k||\Sigma_X||_2}}{\max \mathcal{P}}}{ 1-\frac{1}{\max \mathcal{P}} \sqrt{\frac{\delta^2}{\epsilon} + ||\Sigma_X||_2}} \\
        & \approx \frac{\exp \left(- \frac{ \sqrt{k ||\Sigma_X||_2}}{\max \mathcal{P}}  \right)}{\exp \left(-\frac{1}{\max \mathcal{P}} \sqrt{\frac{\delta^2}{\epsilon} + ||\Sigma_X||_2}\right)}\\
        &=  \exp\left(-\frac{1}{\max \mathcal{P}}  \left( \sqrt{k ||\Sigma_X||_2} - \sqrt{\frac{\delta^2}{\epsilon} + ||\Sigma_X||_2} \right)\right) \\
       & =  \exp\left(-\frac{1}{\max \mathcal{P}}  \left( \sqrt{k ||\Sigma_X||_2} - \sqrt{\frac{20 ||\Sigma_X||_2}{\epsilon} + ||\Sigma_X||_2} \right)\right) \\
       & =  \exp\left(-\frac{1}{\max \mathcal{P}}  \left( \sqrt{ ||\Sigma_X||_2} \left( \sqrt{k} - \sqrt{\frac{20 }{\epsilon} + 1} \right)\right) \right)
    \end{split}
    \end{equation}
    Substituting this into (\ref{eqn:ri_ri-1}) completes the proof. 
\end{proof}

\begin{lemma} \label{lemma:k}
    For $\IE[r_i | r_{i-1}] \leq r_{i-1}$ to hold, a sufficient condition 
    is that $k > \frac{20}{\epsilon}+ 1$, where $k$ is defined in 
    (\ref{eqn:outlier_o})
\end{lemma}
\begin{proof}
    This is a direct consequence of (\ref{equation:ratio}) in Lemma \ref{lemma:ri}. Since $\frac{\sqrt{||\Sigma_X||_2}}{\max \mathcal{P}} > 0$,
    a sufficient condition for $\IE[r_i | r_{i-1}] \leq r_{i-1}$ is $\sqrt{k}- \sqrt{\frac{20}{\epsilon} + 1} > 0$, or equivalently, $k > \frac{20}{\epsilon}+ 1$.  
\end{proof}

\begin{lemma} \label{lemma:tau_r}
    Let $\tau$ be the number of iterations taken by 
    Algorithm \ref{alg:filter_modified}. Then, 
    $$\IE[r_{\tau} |r_0] \leq \frac{2\epsilon}{1-2\epsilon}\exp\left(-\frac{\tau}{30 }   \left( \sqrt{k} - \sqrt{\frac{20 }{\epsilon} + 1} \right)\right) $$
    with a probability of at least $1 - \frac{1}{900}$.
\end{lemma}
\begin{proof}
    By Corollary \ref{corr:maxp}, $\max \mathcal{P} \leq 30 \sqrt{||\Sigma_X||_2}$ with a probability of at least $1 - \frac{1}{900}.$
    Furthermore, by Assumption \ref{assumption:extreme}, any extreme outliers have thus been filtered out. Therefore, the bound in (\ref{eqn:ri_ri-1}) from Lemma \ref{lemma:ri}  becomes
    \[
    \IE[r_{i}|r_{i-1}] \leq r_{i-1} \exp\left(-\frac{1}{30}  \left(\sqrt{k}- \sqrt{\frac{20}{\epsilon} + 1} \right) \right)
    \]
    with a probability of at least $1 - \frac{1}{900}$.
    By the law of total expectation, 
    \[
    \begin{split}
        \IE[r_\tau | r_0] &= \IE[\IE[r_\tau|r_{\tau-1}] | r_0] \\
        & \leq \IE \left[r_{\tau-1}\exp\left(-\frac{1}{30}   \left( \sqrt{k} - \sqrt{\frac{20 }{\epsilon} + 1} \right)\right)\middle| r_0\right].
    \end{split}
    \]
    Repeating this procedure a further $\tau-1$ times, 
    we have
    \begin{equation} \label{eqn:r_tau_r_0}
        \IE[r_\tau | r_0] \leq r_0 \exp\left(-\frac{\tau}{30}   \left( \sqrt{k} - \sqrt{\frac{20 }{\epsilon} + 1} \right)\right).
    \end{equation}
    By Lemma \ref{lemma:2eps}, since $|O_0| \leq 2n\epsilon$,
    \[
        r_0 = \frac{|O_0|}{|I_0|} \leq \frac{2n\epsilon}{n - 2n\epsilon} = \frac{2\epsilon}{1 -2\epsilon},
    \]
    substituting this bound into (\ref{eqn:r_tau_r_0})
    completes the proof. 
\end{proof}

% Lemma \ref{lemma:max_p_bound} describes the relationship between $\max \mathcal{P}$ (defined in Line 8, Algorithm \ref{alg:filter_modified}) and $||\Sigma_X||_2$ (the variance computed across the samples) while Algorithm \ref{alg:filter_modified} has not terminated. 
% \begin{lemma} \label{lemma:max_p_bound}
%     Suppose Algorithm \ref{alg:filter_modified} has not yet terminated. Then, $\sqrt{||\Sigma_X||_2} \leq \max \mathcal{P}$.
% \end{lemma}

% \begin{proof} 
% Let $X_i$ and $u$ be the samples remaining and dominant eigenvector (as given in Line 2 of Algorithm \ref{alg:filter_modified})  in a given iteration.

%     Suppose Algorithm \ref{alg:filter_modified} has not terminated,  then the condition in Algorithm \ref{alg:filter_modified} (Line 9) has not yet been satisfied.  Thus, less than $1-2\epsilon$ proportion of samples in $X_i$  satisfy $p_i / \max \mathcal{P} > 0.5$, where $p_i$ is defined in Line 9 of  Algorithm \ref{alg:filter_modified}. Thus, 
%     \[
%     \begin{split}
%     ||\Sigma_{X_i}||_2& = \frac{1}{|X_i|}\sum_{x \in X_i} |u \cdot (x - \mu_{X_i}) |^2 \\
%     &\leq (1-2\epsilon)\left(\frac{\max \mathcal{P}}{2} \right)^2 + 2\epsilon (\max \mathcal{P})^2 \\
%     & = (\max \mathcal{P})^2 \left( \frac{1}{4}+ \frac{3}{2}\epsilon \right)\\
%     & \leq (\max \mathcal{P})^2,
%     \end{split}
%     \]
%     for all $0 \leq \epsilon \leq \frac{1}{2}$. Hence, $\sqrt{||\Sigma_{X_i}||_2} \leq \max \mathcal{P}$. Since $\sqrt{||\Sigma_{X}||_2} \leq \sqrt{||\Sigma_{X_i}||_2}$, due to the fact that the uncorrupted set $X$ has a variance upper bounded by the variance of the corrupted set $X_i$, 
%     \[
%     \sqrt{||\Sigma_{X}||_2} \leq \sqrt{||\Sigma_{X_i}||_2} \leq \max \mathcal{P},
%     \]
%     and the claim in the lemma follows. 
% \end{proof}

Our goal is now to derive $k$ in (\ref{eqn:outlier_o}), such that  the ratio of the number of outliers to the number of inliers in Lemma \ref{lemma:ri} decreases on expectation in each successive iteration. Lemma \ref{lemma:choice_k} shows that when $k$ takes on certain values, then this ratio decreases in expectation. Corollary \ref{corr:f} sets $k = \left(\sqrt{\frac{20 }{\epsilon} + 1} + \frac{150}{n\epsilon} \right)^2$, and show that for this choice of $k$, the expected ratio of number of inlier samples to the number of outlier samples at the end of $2n\epsilon$ iterations is upper bounded by $\frac{2\epsilon}{1-2\epsilon}\exp(10)$.
\begin{lemma} \label{lemma:choice_k} 
    Let $k \geq \left( -\frac{30}{2n\epsilon} \log f + \sqrt{\frac{20}{\epsilon}+1}    \right)^2$ for some predetermined $0<f<1$. 
    Then, at the end of $\tau = 2n\epsilon$ iterations, $\IE[r_{\tau}|r_0] \leq \frac{2\epsilon}{1-2\epsilon} f$ with a probability lower bounded by $1 - \frac{1}{900}$. 
\end{lemma}
\begin{proof}
    By Lemma \ref{lemma:tau_r}, 
    $$\IE[r_{\tau} |r_0] =\IE\left[\frac{|O_\tau|}{|I_\tau|} \middle| r_0\right] \leq \frac{2\epsilon}{1-2\epsilon}\exp\left(-\frac{\tau}{30 }   \left( \sqrt{k} - \sqrt{\frac{20 }{\epsilon} + 1} \right)\right), $$
    with probability lower bounded by $1-\frac{1}{900}$.
    It therefore suffices to bound
    \begin{equation} \label{eqn:bound_f}
       \exp\left(-\frac{\tau}{30 }   \left( \sqrt{k} - \sqrt{\frac{20 }{\epsilon} + 1} \right)\right)   \leq f.
    \end{equation}
    Taking $\log$ on both side, 
    \[
        -\frac{\tau}{30 }   \left( \sqrt{k} - \sqrt{\frac{20 }{\epsilon} + 1} \right) \leq \log f, 
    \]
    or equivalently, 
    \[
      \sqrt{k} \geq -\frac{30}{\tau} \log f + \sqrt{\frac{20}{\epsilon}+1}.
    \]
    Squaring both sides and substituting $\tau = 2n\epsilon$ yields the required bound on $k$.
\end{proof}

\begin{corollary} \label{corr:f}
    Set $f = \exp(-10)$ and 
    $k = \left(\sqrt{\frac{20 }{\epsilon} + 1} + \frac{150}{n\epsilon} \right)^2.$
    If Algorithm \ref{alg:filter_modified} runs for $\tau=2n\epsilon$ iterations, $\IE[r_\tau|r_0] \leq \frac{2\epsilon}{1-2\epsilon}\exp(-10)$ with a probability lower bounded by $1 - \frac{1}{900}$.
\end{corollary}
\begin{proof}
        The bound for $\IE[r_\tau|r_0]$ can be verified by substituting $f = \exp(-10)$ in Lemma \ref{lemma:choice_k}. 
\end{proof}

% Corollary \ref{corr:remaining} states that at the end of Algorithm \ref{alg:filter_modified}, each outlier sample is expected to be accompanied by at least $\exp(10) \left(\frac{1}{2\epsilon}-1\right)$ inlier samples. With this observation, Corollary \ref{corr:min_bias} shows that for the remaining outlier samples to bias the sample mean by $\delta$ in a given direction, it must deviate from
% the sample mean in this direction by at least $\left(1+\exp(10) \left(\frac{1}{2\epsilon}-1\right)\right) \delta$
% \begin{corollary} \label{corr:remaining}

%     Continuing from Corollary \ref{corr:f}, after $\tau = 2n\epsilon$ iterations, $\IE_0[|I_\tau|] \geq \left(\exp(10) \left(\frac{1}{2\epsilon}-1\right)\right) \IE_0[|O_\tau|]$. In other words, for every remaining outlier, the expected number of remaining inliers increases by at least
%     $\exp(10) \left(\frac{1}{2\epsilon}-1\right)$.
% \end{corollary}
% \begin{proof}
%     This is an immediate consequence of Corollary \ref{corr:f}. 
%      First, note that $\IE[r_\tau|r_0] = \IE_0 \left[\frac{|O_0|}{|I_0|} \frac{A'_\tau}{B'_\tau}\right] = \frac{|O_0| \IE_0[A'_\tau]}{|I_0| \IE_0[B_\tau']},$ where the final equality is due to the independence between the random variables $A_\tau'$ and $B_\tau'$. 
     
%      Since $\IE_0[|O_0| 
%  A'_\tau] = \IE_0[|O_\tau|] $ and $\IE_0[|I_0| 
%  B'_\tau] = \IE_0[|I_\tau|]$, we have $\IE[r_\tau|r_0] = \frac{\IE_0[|O_\tau|]}{\IE_0[|I_\tau|]}$. Thus, $\frac{\IE_0[|O_\tau|]}{\IE_0[|I_\tau|]} \leq  \frac{2\epsilon}{1-2\epsilon}\exp(-10)$, or equivalently, $$\IE_0[|I_\tau|] \geq \exp(10) \frac{1-2\epsilon} {2\epsilon}\IE_0[|O_\tau|] = \left(\exp(10) \left(\frac{1}{2\epsilon}-1\right)\right)\IE_0[|O_\tau|] $$.
% \end{proof}

\begin{corollary} \label{corr:min_bias}
    Let $O_{\tau}$ be the outlier samples that remain after $\tau = 2n\epsilon$ iterations. For the samples in $O_{\tau}$ to bias $\mu_{X_\tau}$ by more than $\delta$ in some direction $v$, a necessary condition is that for all $x \in O_\tau$, $|v\cdot(x - \mu_{I_\tau})| \geq  \left(1+\exp(10) \left(\frac{1}{2\epsilon}-1\right)\right) \delta$, on expectation. 
\end{corollary}
\begin{proof}
    This is a consequence of Corollary \ref{corr:f}. The expected ratio between the number of outlier samples to inlier samples (conditional on $r_0$) admits an upper bound of
    $\IE[r_\tau|r_0] = \IE\left[ \frac{|O_\tau|}{|I_\tau|} \middle| r_0\right] \leq \frac{2\epsilon}{1-2\epsilon}\exp(-10)$. Hence, 
    each $x \in O_\tau$  is expected to be accompanied by at least $N:=\exp(10) \left(\frac{1}{2\epsilon}-1\right)$ inlier samples. Let $S_x$ consist of the outlier sample $x\in O_\tau$ and its accompanying set of inlier samples $\mathcal{I}_x$, where $|\mathcal{I}_x| = N$. Then, for $x$ to bias $\mu_{S_x}$ by at least $\delta$ in a direction $v$ away from $\mu_{\mathcal{I}_x}$, 
    \[
        v \cdot(\mu_{S_x} - \mu_{\mathcal{I}_x}) = \frac{1}{N+1} \left(  v \cdot(x - \mu_{\mathcal{I}_x}) + \sum_{i \in \mathcal{I}_x} v \cdot(i - \mu_{\mathcal{I}_x}) \right) \geq \delta.
    \]
    A necessary condition is thus, 
    \[
        \frac{1}{N+1} \left(  v \cdot(x - \mu_{\mathcal{I}_x}) \right) \geq \delta,
    \]
    or equivalently, 
    \[
         v \cdot(x - \mu_{\mathcal{I}_x})  \geq (N+1)\delta. 
    \]
\end{proof}
    
\begin{corollary} \label{corr:ei}
    Set 
    $k =  \left(\sqrt{\frac{20 }{\epsilon} + 1} + \frac{150}{n\epsilon} \right)^2$,
    and let $\epsilon'_i$ be as defined in (\ref{eqn:ei}). Then,
    \[
        \IE[\epsilon_i' | r_0] \leq \frac{1}{1 + \frac{1-2\epsilon}{2\epsilon} \exp\left( i \frac{60}{n}\right)},
    \]
    with probability of at least $1 - \frac{1}{900}$. Hence, $\IE[\epsilon_\tau' | r_0] \approx 0$.

\end{corollary}
\begin{proof}
    Substituting our choice of $k$ in Lemma \ref{lemma:tau_r}, we obtain:
    \[
            \begin{split}
        \IE[r_{i} |r_0] & \leq \frac{2\epsilon}{1-2\epsilon}\exp\left(-\frac{i}{30 }   \left( \sqrt{\frac{20 }{\epsilon} + 1} + \frac{150}{n\epsilon} - \sqrt{\frac{20 }{\epsilon} + 1} \right)\right) \\
        &= \frac{2\epsilon}{1-2\epsilon} \exp\left( - i \frac{5}{n\epsilon}\right) \\
        & \leq  \frac{2\epsilon}{1-2\epsilon} \exp\left( - i \frac{60}{n}\right),
    \end{split}
    \]
    where the final inequality is due to $\epsilon \leq \frac{1}{12}$.
    Since 
    \[
        \epsilon_{i}' = \left( \frac{|O_i| + |I_i|}{|O_i|}\right) ^{-1} = \left( 1 + \frac{1}{r_i}\right) ^{-1},
    \]
    we have
    \[
        \begin{split}
            \IE[\epsilon_i' | r_0] &= \IE \left[ \left( 1 + \frac{1}{r_i}\right) ^{-1} \middle| r_0\right] \\
            & \leq \left( 1 + \left(\frac{2\epsilon}{1-2\epsilon} \exp\left( - i \frac{60}{n}\right) \right)^{-1} \right)^{-1} \\
            &= \frac{1}{1 + \frac{1-2\epsilon}{2\epsilon} \exp\left( i \frac{60}{n}\right)},
        \end{split}
    \]
    as required.   
\end{proof}

Lemma \ref{lemma:sigma_xi_decreasing} relates the stopping condition in Line 3 of Algorithm \ref{alg:filter_modified} (i.e. the convergence of the eigenvalues computed over successive iterations) to the convergence of the sample covariance matrix $||\Sigma_{X_\tau}||_2$ to the covariance matrix over the inlier samples $||\Sigma_{I_\tau}||_2$. Subsequently, Lemma 
\ref{lemma:line3} shows that if this convergence condition is met, the  proportion of outlier samples (w.r.t. the total number of remaining samples) is close to 0. 
\begin{lemma}\label{lemma:sigma_xi_decreasing}
    Suppose Algorithm \ref{alg:filter_modified} terminates at $\tau \leq 2n\epsilon$
    iterations, and $k =  \left(\sqrt{\frac{20 }{\epsilon} + 1} + \frac{150}{n\epsilon} \right)^2$. Then, the sequence of values $\IE_0[||\Sigma_{X_i}|| - ||\Sigma_{I_i}||_2]$ converges to 0, for $i=1, \dots, \tau$, with probability of at least $1 - \frac{1}{900}$. 
    
\end{lemma}

\begin{proof}
        The following is an algebraic fact (also used in the original analysis of~\cite{diakonikolas2023algorithmic})):
    \begin{equation} \label{eqn:sigma_xi}
        \Sigma_{X_i} = (1-\epsilon'_i) \Sigma_{I_i} + \epsilon'_i \Sigma_{O_i} + \epsilon'_i (1-\epsilon'_i) (\mu_{O_i} - \mu_{I_i})(\mu_{O_i} - \mu_{I_i})^T,
    \end{equation}
    By Corollary \ref{corr:ei}, the sequence of values $\IE[\epsilon'_i|\epsilon'_0]$ is exponentially decreasing in $i$, and converges to 0 as $i$ increases. Thus, the terms in (\ref{eqn:sigma_xi}) which are proportional to $\epsilon_i'$ are decreasing and converging to 0
    in expectation, while $(1-\epsilon'_i) \Sigma_{I_i}$ is converging to $\Sigma_{I_i}$. Thus, 
    $\Sigma_{X_i}$ is converging to $\Sigma_{I_i}$. Hence, $\IE_0[||\Sigma_{X_i}||_2 - ||\Sigma_{I_i}||_2]$ 
    % Finally, at iteration $\tau$, since $|O_\tau|=0$, the sequence is no longer decreasing. 
\end{proof} 

\begin{lemma} \label{lemma:line3}
    Suppose Algorithm \ref{alg:filter_modified} terminates at $\tau < 2n\epsilon$ iterations at Line 3. Then, $\epsilon'_\tau \approx 0$, and 
    $\IE[\epsilon_i' | r_0] \leq \frac{1}{1 + \frac{1-2\epsilon}{2\epsilon} \exp\left( i \frac{60}{n}\right)}$ with probability at least $1-\frac{1}{900}$.
\end{lemma}
\begin{proof}
    Suppose $\epsilon'_\tau \not \approx 0$. By Corollary \ref{corr:ei}, the expectation of $\epsilon_i'$, conditional on $r_0$ is
    \[
    \IE[\epsilon_i' | r_0] \leq \frac{1}{1 + \frac{1-2\epsilon}{2\epsilon} \exp\left( i \frac{60}{n}\right)}
    \]
    This expectation decreases exponentially with the number of iterations with probability at least $1-\frac{1}{900}$,  and is lower bounded by 0. Thus, if $\epsilon'_\tau \not \approx 0$, the sequence $||\Sigma_{X_i}||_2 - ||\Sigma_{I_i}||_2$ in Lemma \ref{lemma:sigma_xi_decreasing} has not converged in expectation, and the condition in Line 3 of Algorithm \ref{alg:filter_modified} has not been satisfied. 
\end{proof}


Finally, in Theorem \ref{thm:bias_revised}, we formally prove our claim that if $X_\tau$ is the samples remaining after Algorithm \ref{alg:filter_modified} has terminated, then, the maximum bias of $X_\tau$ (w.r.t. the set of clean samples $S$) in any direction  is upper bounded by $\delta$.
\begin{theorem*} [\emph{Theorem \ref{thm:bias_revised} restated}]
    Let $S$ be a $(\epsilon, \delta)$-stable set, where $\epsilon \leq 1/12$, 
    $\delta = \sqrt{20 ||\Sigma_S||_2}$, and $X$ is an $\epsilon$-corrupted
    version of $S$, and let $k =  \left(\sqrt{\frac{20 }{\epsilon} + 1} + \frac{150}{n\epsilon} \right)^2$. 
    Suppose Algorithm \ref{alg:filter_modified} terminates after $\tau \leq 2n\epsilon$
     number of iterations. Let $X_\tau$ be the samples remaining after $\tau$ iterations. Then, for any unit vector $v$, $|v \cdot (\mu_{X_\tau} - \mu_S)| \leq \delta$ with probability of at least $1-\frac{1}{900}$. 
    %, assuming Algorithm~\ref{alg:filter_original} is a strong aggregator.
\end{theorem*}
\begin{proof} %[\emph{Revised Proof}]
    Let  $X_i$ denote the remaining points in $X$ at the start of the $i$-th iteration, $\epsilon'_i$ denote
    the proportion of outliers (as defined in (\ref{eqn:ei}). Let $\tau$ be the number of iterations taken by Algorithm \ref{alg:filter_modified}. To evaluate its correctness, we analyze all the $3$ stopping conditions:
    \begin{enumerate}
        \item Algorithm \ref{alg:filter_modified} terminates at $\tau=2n\epsilon$ iterations. By Lemma  \ref{lemma:2eps}, there are at most $|O_0| \leq 2n\epsilon$ outliers. Since each iteration removes at least one outlier sample, all samples in $O_0$ will be removed at the end of $2n\epsilon$ iterations. 
        \item Algorithm \ref{alg:filter_modified} terminates at Line 3 for some iteration $\tau < 2n\epsilon$. By Lemma \ref{lemma:line3}, if the condition in Line 3 is fulfilled, $\epsilon_\tau' \approx 0$. For contradiction, assume $|O_\tau| > 0$. Then, by Corollary \ref{corr:min_bias}, for $O_\tau$ to bias $\mu_{X_\tau}$ away from $\mu_{I_\tau}$ by $\delta$ in some direction $v$, each  sample $x \in O_\tau$ must introduce a bias of  
        \[
        \begin{split}
        v\cdot(x - \mu_{I_\tau}) & \geq \left(1+\exp(10) \left(\frac{1}{2\epsilon}-1\right)\right) \delta\\
        & = \left(1+\exp(10) \left(\frac{1}{2\epsilon}-1\right)\right)  \sqrt{20 ||\Sigma_S||_2}\\
        & \geq \left(1+5\exp(10)\right)  \sqrt{20 ||\Sigma_S||_2} \\
        & \geq 30 \sqrt{||\Sigma_S||_2}
        \end{split}
        \]
        where the second last inequality is due to $\epsilon \leq \frac{1}{12}$.
        By our Assumption \ref{assumption:extreme}, such extreme outliers would have been removed in the pre-processing step itself. Thus, $|O_\tau| = 0$. 
        % However, if such an extreme outlier exists, the convergence of $||\Sigma_{X_i}||_2 - ||\Sigma_{I_i}||_2$ in Lemma \ref{lemma:sigma_xi_decreasing} will not be satisfied, as removing this outlier will result in a significant 
        % decrease in $||\Sigma_{X_\tau}||_2$. Thus, $|O_\tau| = 0$. By the stability of $S$, $|v\cdot(\mu_{X_\tau} - \mu_S)| \leq \delta$
        \item If Algorithm \ref{alg:filter_modified} terminates due to Line 9 for some iteration $\tau < 2n\epsilon$, then $|O_\tau| = 0$. For contradiction suppose that $|O_\tau| > 0$. Then, by Corollary \ref{corr:min_bias}, for $O_\tau$ to bias $\mu_{X_\tau}$ away from $\mu_{I_\tau}$ by $\delta$ in some direction $v$, each  sample $x \in O_\tau$ must introduce a bias of $v\cdot(x - \mu_{I_\tau})   \geq \left(1+5\exp(10)\right)  \sqrt{20 ||\Sigma_S||_2}$. Thus, 
        \begin{equation} \label{eqn:maxp_line9}
        \max \mathcal{P} \geq \left(1+5\exp(10)\right)  \sqrt{20 ||\Sigma_S||_2}
        \end{equation}
        and thus, for a proportion at least $1 - 2\epsilon = \frac{5}{6}$ samples in $X_\tau$,
        \[
        \begin{split}
            p_i& \geq \frac{1}{2} \max \mathcal{P} \\
            & \geq \frac{1}{2} \left(1+5\exp(10)\right)  \sqrt{20 ||\Sigma_S||_2}\\
            & \geq 30 \sqrt{||\Sigma_S||_2}.
        \end{split}
        \]
        But, by our Assumption \ref{assumption:extreme}, such extreme outliers would have been removed in the preprocessing step. Thus, $|O_\tau| = 0$.
    \end{enumerate}
    In all the 3 stopping conditions of the algorithm, we showed that $|O_\tau| = 0$. Hence by the $(\epsilon, \delta)$-stability condition of $S$ (Definition \ref{dfn:epsilon_delta_stable} (1)), for any unit vector $v$, $|v \cdot (\mu_{X_\tau} - \mu_S)| \leq \delta$ for $X_{\tau}$ that remains.
\end{proof}

